Benchmarking Attacks on Learning with Errors

Lattice cryptography schemes based on the learning with errors (LWE) hardness assumption have been standardized by NIST for use as post-quantum cryptosystems, and by HomomorphicEncryption.org for encrypted compute on sensitive data. Thus, understanding their concrete security is critical. Most work on LWE security focuses on theoretical estimates of attack performance, which is important but may overlook attack nuances arising in real-world implementations. The sole existing concrete benchmarking effort, the Darmstadt Lattice Challenge, does not include benchmarks relevant to the standardized LWE parameter choices - such as small secret and small error distributions, and Ring-LWE (RLWE) and Module-LWE (MLWE) variants. To improve our understanding of concrete LWE security, we provide the first benchmarks for LWE secret recovery on standardized parameters, for small and low-weight (sparse) secrets. We evaluate four LWE attacks in these settings to serve as a baseline: the Search-LWE attacks uSVP, SALSA, and Cool & Cruel, and the Decision-LWE attack: Dual Hybrid Meet-in-the-Middle (MitM). We extend the SALSA and Cool & Cruel attacks in significant ways, and implement and scale up MitM attacks for the first time. For example, we recover hamming weight $9-11$ binomial secrets for KYBER ($\kappa=2$) parameters in $28-36$ hours with SALSA and Cool\&Cruel, while we find that MitM can solve Decision-LWE instances for hamming weights up to $4$ in under an hour for Kyber parameters, while uSVP attacks do not recover any secrets after running for more than $1100$ hours. We also compare concrete performance against theoretical estimates. Finally, we open source the code to enable future research.

==> figures/functions.tex <==
\begin{figure*}[t]
\begin{python}
    def SparseDiscreteGaussian(stddev, mean=0, n=None, h=None):
        # Discrete Gaussian with standard deviation ``stddev`` per component and fixed Hamming h.
        b_val = oo if n is None else ceil(log(n, 2) * stddev)
        if h == None:
            density = 1 - min(RR(1 / (sqrt(2 * pi) * stddev)), 1.0)
        else:
            density = RR(h/n)
        return NoiseDistribution(stddev=RR(stddev), mean=RR(mean), n=n, bounds=(-b_val, b_val), 
        density=density, tag="SparseDiscreteGaussian")
\end{python}
\begin{python}
 def SparseCenteredBinomial(eta, n=None, h=None):
        # Sample a_1, ..., a_eta, b_1, ..., b_eta and return sum(a_i - b_i). If h!=None, zero out out all but h components.
        stddev = sqrt(eta / 2.0)
        if h == None:
            density = 1 - binomial(2 * eta, eta) * 2 ** (-2 * eta)
        else:
            density = RR(h/n)
        return NoiseDistribution(stddev=RR(stddev), density=density, mean=RR(0), n=n, 
        bounds=(-eta, eta), tag="SparseCenteredBinomial")
\end{python}
\vspace{-0.1cm}
\caption{Code added to \texttt{nd.py} in Lattice Estimator to support sparse Gaussian and binomial secrets.}
\label{fig:functions}
\end{figure*}

==> tables/he_bench.tex <==
\begin{table}[t]
\centering

\begin{tabular}{cclccc}
\toprule
$n$ & $\log_2 q$ & $q$ & $X_s$ & $X_e$  \\ \midrule % & $h$
1024 & 26 & 41223389 & $\ternsech$ & $\normsec$  \\[0.2cm]
1024 & 29 & 274887787 &  $\ternsech$ & $\normsec$  \\[0.2cm]
1024 & 50 & 607817174438671 & $\ternsech$ & $\normsec$  \\ \bottomrule
\end{tabular}
\caption{Proposed benchmark settings for HE. $\sigma=3.19$ for both $X_e$ and $X_s = \normsech$ (where appropriate). All settings use Ring-LWE.}
\label{tab:he_bench}
\vspace{-0.2cm}
\end{table}


==> tables/he_estimates.tex <==
\begin{table*}[]
\begin{tabular}{llllllllllllll}

\toprule
\multirow{2}{*}{$n$} & \multirow{2}{*}{$\log_2 q$} & \multirow{2}{*}{$h$} & \multirow{2}{*}{cost model} \hspace{0.3cm} & \multicolumn{3}{c}{USVP} \hspace{0.4cm} & \multicolumn{7}{c}{Dual Hybrid MiTM} \\ \cmidrule{5-14}
 &  &  &  & ROP & time (yrs) & BKZ $\beta$ \hspace{0.4cm} & ROP & repeats & time & memory & $\tau$ & $\zeta$ & $h_1$ \\ \midrule



% logq 26 with SPARSE TERNARY
 \multirow{3}{*}{1024} & \multirow{3}{*}{26} & \multirow{3}{*}{7} & CheNgu12 & $2^{200.2}$ & 2.75e43 & 309 & $2^{39.7}$ & $2^{8.0}$ & 31 hrs & $2^{29.5}$ (3 GB) & 255 & 883 & 5 \\
 &  &  & ABLR21 & $2^{163.0}$ & 1.7e32 & 309 & $2^{45.9}$ & $2^{7.3}$ & 58 days & $2^{33.1}$ (40 GB) & 211 & 952 & 6 \\
 &  &  & MATZOV & $2^{118.1}$ & 5.4e18 & 309 & $2^{45.6}$ & $2^{7.4}$ & 51 days & $2^{33.1}$ (40 GB) & 203 & 960 & 6 \\ \midrule %\cmidrule{4-14}

 % logq 29
\multirow{3}{*}{1024} & \multirow{3}{*}{29} & \multirow{3}{*}{11} & CheNgu12 & $2^{244.9}$ & 8.1e56 & 363 & $2^{45.2}$ & $2^{10.8}$ & 1.1 yrs & $2^{34.7}$ (100 GB) & 314 & 828 & 6 \\
 &  &  & ABLR21 & $2^{194.3}$ & 4.8e41 & 363 & $2^{49.2}$ & $2^{9.5}$ & 7.4 yrs & $2^{38.7}$ (1.8 TB) & 300 & 839 & 7 \\
 &  &  & MATZOV & $2^{133.4}$ & 2.2e23 & 363 & $2^{48.9}$ & $2^{9.1}$ & 4.4 yrs & $2^{38.6}$ (1.6 TB) & 305 & 820 & 7 \\ \midrule

 % logq 34
\multirow{3}{*}{1024} & \multirow{3}{*}{34} & \multirow{3}{*}{13} & CheNgu12 & $2^{170.7}$ & 3.8e34 & 271 & $2^{45.6}$ & $2^{11.4}$ & 2.3 yrs & $2^{33.7}$ (100 GB) & 397 & 759 & 6 \\
 &  &  & ABLR21 & $2^{142.4}$ & 1.1e26 & 271 & $2^{50.1}$ & $2^{9.9}$ & 17.3 yrs & $2^{38.6}$ (1.6 TB) & 385 & 758 & 7 \\
 &  &  & MATZOV & $2^{108.0}$ & 4.9e15 & 271 & $2^{49.6}$ & $2^{9.8}$ & 11.3 yrs & $2^{37.7}$ (0.9 TB) & 386 & 750 & 7 \\ \midrule

 % logq 45
\multirow{3}{*}{1024} & \multirow{3}{*}{45} & \multirow{3}{*}{18} & CheNgu12 & $2^{100.6}$ & 3.0e13 & 172 & $2^{46.9}$ & $2^{11.4}$ & 5.1 yrs & $2^{33.7}$ (100 GB) & 564 & 589 & 6 \\
 &  &  & ABLR21 & $2^{93.0}$ & 1.5e11 & 172 & $2^{51.0}$ & $2^{9.7}$ & 28.1 yrs & $2^{40.7}$ (7.0 TB) & 550 & 613 & 8 \\
 &  &  & MATZOV & $2^{80.7}$ & 3.0e7 & 172 & $2^{50.7}$ & $2^{10.1}$ & 32.0 yrs & $2^{39.7}$ (3.5 TB) & 531 & 634 & 8 \\ \midrule

 
\multirow{3}{*}{1024} & \multirow{3}{*}{50} & \multirow{3}{*}{18} & CheNgu12 & $2^{83.4}$ & 1.9e8 & 144 & $2^{45.7}$ & $2^{9.9}$ & 0.8 & $2^{33.6}$ (50 GB) & 623 & 523 & 6 \\
 &  &  & ABLR21 & $2^{80.8}$ & 3.1e7 & 144 & $2^{49.9}$ & $2^{9.0}$ & 8.1 & $2^{39.7}$ (3.5 TB) & 612 & 557 & 8 \\
 &  &  & MATZOV & $2^{73.1}$ & 1.5e5 & 144 & $2^{49.7}$ & $2^{9.1}$ & 7.6 & $2^{37.6}$ (800 GB) & 597 & 525 & 7 \\ \bottomrule
\end{tabular}
\caption{{\bf Estimated performance of uSVP and Dual Hybrid MiTM attacks on Homomorphic Encryption benchmark settings.} According to Estimator documentation, ``ROP'' approximates the number of CPU cycles needed to run the attack, so we convert to time by dividing this by 2.1GHz ($2.1e9$ cycles/sec), the clock speed of our CPUs. For Dual Hybrid, we multiply this by estimated repeats, the number of times the attack must run to succeed with probability $0.99$. We convert predicted memory to bytes by multiplying estimator output (number of integers to be stored) by number of bits required to store this integer (we use $32$).}
\label{tab:he_estimates}
\end{table*}

==> tables/he_summary.tex <==

\begin{table*}[]
\begin{tabular}{clccccc}
\toprule
\multirow{2}{*}{Attack} & \multirow{2}{*}{Results} & \multicolumn{5}{c}{LWE Setting ($n$, $\log_2 q$)} \\ \cmidrule{3-7}
 &  & (1024, 26) & (1024, 29) & (1024, 34) & (1024, 45) & (1024, 50) \\ \midrule
\multirow{5}{*}{uSVP} & Best $h$ &  &  &  &  &  \\
 & Preproc. time &  &  &  &  &  \\
 & Recovery time &  &  &  &  &  \\
 & Success rate &  &  &  &  &  \\
 & Memory &  &  &  &  &  \\ \midrule
\multirow{5}{*}{ML} & Best $h$ (ternary/gaussian) & 8 & 10 / 8 &  &  & 17 / 13 \\
 & Preproc. time & $2^{27.3}$ &$2^{27.8}$  & $2^{25.7}$ &$2^{29.0}$ & $2^{27.4}$ \\
 & Recovery time & $2^{15.56}$ & $2^{15.97}$ &  &  & $2^{14.22}$ \\
 & Success rate & $1/10$ & $1/10$ &  &  & $1/10$ \\
 & Memory &  &  &  &  &  \\ \midrule
\multirow{5}{*}{CC} & Best $h$ (ternary/gaussian) & 7 / NA & 12 / 8 &  &  & 20 / none \\
 & Preproc. time & $2^{22.9}$ & $2^{23.5}$ & $2^{21.4}$ &$2^{24.7}$  & $2^{23.1}$ \\
 & Recovery time & $2^{10.54}$ & $2^{8.88}$ &  &  & $2^{13.87}$ \\
 & Success rate & $2/10$ & $1/10$ &  &  & $2/10$ \\
 & Memory &  &  &  &  &  \\ \midrule
\multirow{5}{*}{MITM} & Best $h$ &  &  &  &  &  \\
 & Preproc. time &  &  &  &  &  \\
 & Recovery time &  &  &  &  &  \\
 & Success rate &  &  &  &  &  \\
 & Memory &  &  &  &  &  \\ \bottomrule
\end{tabular}
\caption{{\bf HE benchmark results.}}
\label{tab:he_summary}
\end{table*}



==> tables/kyber_detailed_all.tex <==
\begin{table}[t]
\resizebox{0.49\textwidth}{!}{
\centering
\begin{tabular}{cccc@{\hskip 0.3in}ccc@{\hskip 0.3in}ccc}
\toprule
\multirow{2}{*}{Attack} & 
\multicolumn{3}{c}{\hspace{-0.2in} $k=2,\;\log q=12$} & \multicolumn{3}{c}{\hspace{-0.2in} $k=2,\;\log q=28$} & \multicolumn{3}{c}{ \hspace{-0.1in} $k=3,\;\log q=35$} \\[0.1cm]
& $h$ & Rate & Time & $h$ & Rate & Time & $h$ & Rate  &  Time \\
\midrule
\multirow{4}{*}{ML} & 
6 & 6 / 10 & $1.2$ & 15 & 5 / 10& $1.2$ & 14 & 2 / 10& $1.2$ \\
& 7 & 1 / 10 & $1.6$ & 16 & 2 / 10& $1.7$ & 15 & 3 / 10& $15.8$ \\
& 8 & 0 / 10 & - & 17 & 1 / 10& $25.7$ & 16 & 1 / 10& $3.7$ \\
& 9 & 1 / 10 & $7.4$ & 18 & 1 / 10& $17$ & 17 & 0 / 10 & - \\
\midrule
\multirow{5}{*}{CC} & 
7 & 10 / 10 & $0.03$ & 19 & 4 / 10 & $0.1$ & 16 & 4 / 10 & $0.03$ \\
& 8 & 7 / 10 & $0.06$ & 20 & 3 / 10 & $0.2$ & 17 & 6 / 10 & $0.1$ \\
& 9 & 6 / 10 & $0.04$ & 21 & 3 / 10 & $0.6$ & 18 & 4 / 10 & $0.03$ \\
& 10 & 1 / 10 & $1.4$ & 24 & 2 / 10 & $1.0$ & 19 & 2 / 10 & $0.9$ \\
& 11 & 2 / 10 & $0.1$ & 25 & 1 / 10 & $41.8$ & 20 & 0 / 10 & - \\
\midrule
\midrule
\multirow{3}{*}{MiTM} & 
4 & 2 / 10 & 0.2 & 11 & 1 / 10& 0.14 & 12 & 1 / 10& 19 \\
& 5 & 0 / 10 & - & 12 & 1 / 10&  0.02 & 13 & 2 / 10&   15  \\
& 6 & 0 / 10 & - & 13 & 0 / 10& - & 14 & 1 / 10& 25 \\
%9 & 1 / 10 & $2^{22.7}$ & 18 & 1 / 10& $2^{23.9}$ & 17 & 0 / 10 & - \\
\bottomrule
\end{tabular}
}
\caption{{\bf Detailed attack results on Kyber benchmark settings for varying $h$, $n=256$ for all, binomial secrets.} Rate = secrets recovered / attempted. Time = in hours, best single CPU/GPU time for recovering secrets via model training/brute force/MiTM table queries. Required compute resources are given in Table~\ref{tab:all_results}. Preprocessing/short vector generation time is the same for all $h$ at a given setting and is listed as Multi-CPU hrs in Table~\ref{tab:all_results}. }
\label{tab:kyber_detailed_all}
\end{table}

==> tables/kyber_estimates.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{llllllllllllll}
\toprule
\multirow{2}{*}{$n$} & \multirow{2}{*}{$\log_2 q$} & \multirow{2}{*}{$h$} & \multirow{2}{*}{cost model} \hspace{0.3cm} & \multicolumn{3}{c}{USVP} \hspace{0.4cm} & \multicolumn{7}{c}{Dual Hybrid MITM} \\ \cmidrule{5-14}
 &  &  &  \hspace{0.3cm} & ROP & time (yrs) & BKZ $\beta$ \hspace{0.4cm} & ROP & repeats & time (yrs) & memory & $\tau$ & $\zeta$ & $h_1$ \\ \midrule

 % 512 12
\multirow{3}{*}{512} & \multirow{3}{*}{12} & \multirow{3}{*}{10} & CheNgu12~\cite{CN11_BKZ} & $2^{260.0}$ & $2.8e61$ & 382 & $2^{49.4}$ & $2^{15.3}$  & $467.7$ & $2^{34.7}$ (100 GB)  & 103 & 482 & 6 \\

 &  &  & ABLR21~\cite{albrecht2021lattice} & $2^{204.5}$ & $5.5e44$ & 382 & $2^{50.3}$ & $2^{11.0}$ & $44.7$ & $2^{39.7}$ (3.5 TB) & 80 & 496 & 8 \\
 
 &  &  & MATZOV~\cite{matzov} & $2^{137.1}$ & $2.9e24$ &382 & $2^{49.0}$ & $2^{9.7}$ & $7.6$ & $2^{39.7}$ (3.5 TB) & 92 & 486 & 8 \\ \cmidrule{4-14}

 % 512 28
\multirow{3}{*}{512} & \multirow{3}{*}{28} & \multirow{3}{*}{19} & CheNgu12 & $2^{62.8}$ & $120$ & 109 & $2^{48.9}$ & $2^{9.2}$ & $4.7$ & $2^{38.7}$ (1.8 TB) & 331 & 274 & 8 \\

 &  &  & ABLR21 & $2^{65.7}$ & $932$ & 109 & $2^{48.9}$ & $2^{9.2}$ & $4.7$ & $2^{38.7}$ (1.8 TB) & 331 & 274 & 8 \\
 
 &  &  & MATZOV & $2^{62.4}$ & $89$ & 109 & $2^{48.9}$ & $2^{9.2}$ & $4.7$ & $2^{38.7}$ (1.8 TB) & 331 & 274 & 8 \\ \cmidrule{4-14}

 % 768 35
\multirow{3}{*}{768} & \multirow{3}{*}{35} & \multirow{3}{*}{17} & CheNgu12 & $2^{81.7}$ &$5.9e7$ & 142 & $2^{49.4}$ & $2^{9.4}$ & $7.6$ & $2^{37.6}$ (800 GB) & 431 & 428 & 7 \\

 &  &  & ABLR21 & $2^{79.4}$ & $1.2e7$  & 142 & $2^{49.4}$ & $2^{9.4}$  & $7.6$ & $2^{37.6}$ (800 GB) & 431 & 428 & 7 \\
 
 &  &  & MATZOV & $2^{72.0}$ & $7.2e4$& 142 & $2^{49.4}$ & $2^{9.4}$  & $7.6$ & $2^{37.6}$ (800 GB) & 431 & 428 & 7 \\ \bottomrule
 
\end{tabular}
\caption{{\bf Estimated performance of uSVP and Dual Hybrid MiTM attacks on Kyber benchmark settings.} According to Estimator documentation, ``ROP'' approximates the number of CPU cycles needed to run the attack, so we convert to time by dividing this by 2.1GHz ($2.1e9$ cycles/sec), the clock speed of our CPUs. For Dual Hybrid, we multiply this by estimated repeats, the number of times the attack must run to succeed with probability $0.99$. We convert predicted memory to bytes by multiplying estimator output (number of integers to be stored) by number of bits required to store this integer (we use $32$).}
\label{tab:kyber_estimates}
\end{table*}

==> tables/kyber_summary.tex <==

% \usepackage{multirow}
\begin{table}[]
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{clccc}
\toprule
\multirow{2}{*}{Attack} & \multirow{2}{*}{Results} & \multicolumn{3}{c}{MLWE Setting ($k$, $\log_2 q$)} \\ \cmidrule{3-5}
%\begin{tabular}[c]{@{}c@{}}LWE Setting\\ ($n$, $\log_2 q$)\end{tabular} &  & (512, 12) & (512, 28) & (768, 35) \\ \hline
 &  & (512, 12) & (512, 28) & (768, 35) \\ \midrule
\multirow{5}{*}{uSVP} & Best $h$ &  &  &   \\
 & Preproc. time   &  &  &  \\
 & Recovery time &  &  &  \\
 & Success rate  &  &  &  \\
 & Memory &  &  &  \\ \midrule
\multirow{5}{*}{ML} & Best $h$ & 9 & 18 & 16 \\
 & Preproc. time (s) (1CPU)& $2^{28.3}$ & $2^{26.8}$ & $2^{27.7}$ \\
 & Recovery time (s) (1GPU)& $2^{22.7}$ & $2^{23.8}$ & $2^{21.7}$ \\
 & Success rate & $1/10$ & $1/10$ & $1/10$ \\
 & Memory &  &  &  \\ \midrule
\multirow{5}{*}{CC} & Best $h$ & 11 & 25 & 19 \\
 & Preproc. time (s) (1CPU)& $2^{23.9}$ & $2^{22.4}$ & $2^{23.4}$ \\
 & Recovery time (s) (1GPU) & $2^{16.1}$ & $2^{25.2} $ & $2^{19.6}$ \\
 & Success rate & $1/10$ & $1/10$ & $2/10$ \\
 & Memory &  &  &  \\ \midrule
\multirow{5}{*}{MITM} & Best $h$ &  &  &  \\
 & Preproc. time  &  &  &  \\
 & Recovery time   &  &  &  \\
 & Success rate  &  &  &  \\
 & Memory  &  &  &  \\ \bottomrule
\end{tabular}
}
\caption{{\bf Kyber benchmark results (draft).} Categories presented per attack: best hamming weight, preprocessing time, recovery time, probability of success, memory used (CC/AI = dataset memory + 32GB GPU). '-' indicates that an attack did not succeed.}
\label{tab:he_summary_alt}
\end{table}

==> tables/mitm_he.tex <==
\begin{table*}[]
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{ccc@{\hskip 0.4in}ccc@{\hskip 0.4in}ccc@{\hskip 0.4in}ccc@{\hskip 0.4in}ccc}
\toprule
\multicolumn{3}{c}{\hspace{-0.2in} $n=1024,\; \log q=26$} & \multicolumn{3}{c}{\hspace{-0.3in} $n=1024,\; \log q=29$} & \multicolumn{3}{c}{\hspace{-0.3in} $n=1024,\; \log q=34$} & \multicolumn{3}{c}{\hspace{-0.3in} $n=1024,\; \log q=45$} & \multicolumn{3}{c}{\hspace{-0.1in} $n=1024,\; \log q=50$} \\
\multicolumn{3}{c}{ternary} & \multicolumn{3}{c}{gaussian} & \multicolumn{3}{c}{gaussian} & \multicolumn{3}{c}{gaussian} & \multicolumn{3}{c}{gaussian} \\ \midrule
$h$ & Rate & Time & $h$ & Rate & Time & $h$ & Rate & Time & $h$ & Rate & Time & $h$ & Rate & Time \\ \midrule
8 & 2 / 10 & 38 & 7 & X / 10 & TBD & X & X / 10  & X & 10 & 1 / 10 & 1 & 11 & TBD / 10 & TBD \\
9 & 1 / 10  & 57 & 9 & 1 / 10 & 2  & X & X / 10 & X & 11 & 1 / 10 & 1.6 & 12 & 1 / 10 & 3 \\
10 & 0 / 10 & - & 10  & 0 / 10 &- & X & X / 10 & X & 12 & 0 / 10 & -  & 13 & 0 / 10 & - \\ \bottomrule
\end{tabular}
}
\caption{\textbf{Detailed DH MiTM HE Attack results for varying $h$.} Rate = number of secrets recovered / attempted. Time = in hours, best single CPU time for MiTM recovery time (short vector generation time listed as Multi-CPU hrs in Table~\ref{tab:all_results}. }
\label{tab:mitm_he_practical}
\end{table*}


==> tables/mitm_kyber.tex <==
\begin{table}[h]
\resizebox{0.49\textwidth}{!}{
\centering
\begin{tabular}{crrl@{\hskip 0.3in}rrl@{\hskip 0.3in}rrl}
\toprule
\multirow{2}{*}{Attack} & 
\multicolumn{3}{l}{$k=2,\;\log Q=12$} & \multicolumn{3}{l}{$k=2,\;\log Q=28$} & \multicolumn{3}{l}{$k=3,\;\log Q=35$} \\ 
& $h$ & Rate & Time & $h$ & Rate & Time & $h$ & Rate  &  Time \\
\midrule
\multirow{3}{*}{MiTM} & 
4 & 2 / 10 & 0.2 & 11 & 1 / 10& 0.14 & 12 & TBD / 10& TBD \\
& 5 & 0 / 10 & - & 12 & 1 / 10&  0.02 & 13 & TBD / 10& TBD \\
& 6 & 0 / 10 & - & 13 & 0 / 10& - & 14 & 1 / 10& 25 \\
%9 & 1 / 10 & $2^{22.7}$ & 18 & 1 / 10& $2^{23.9}$ & 17 & 0 / 10 & - \\
\bottomrule
\end{tabular}
}
\caption{{\bf Detailed DH MiTM Kyber attack results for varying $h$}. Rate = number of secrets recovered / attempted. Time = in hours, best single CPU time for recovering secrets (short vector generation time listed as Multi-CPU hrs in Table~\ref{tab:all_results}. }
\label{tab:mitm_kyber_practical}
\end{table}
